StepKV: Step-Aware KV Cache Compression for LLM Agents

Key-value (KV) caching is essential for efficient autoregressive large language model (LLM) inference, but the cache grows linearly with context length, increasing storage and decoding costs. KV cache compression mitigates this cost by retaining only a subset of cached tokens. This challenge is particularly important for multi-step LLM agents, where a query expands into trajectories of reasoning, tool interactions, and retrieved observations. Existing pruning methods typically treat the cache as a flat token stream and rank tokens by recency or attention saliency. This creates a mismatch between the unit of compression and the unit of reasoning: token-level pruning removes individual entries, whereas useful information in multi-step agents is often organized into reasoning steps with uneven and delayed importance. Consequently, an early observation or intermediate decision may receive little recent attention yet remain essential for later evidence synthesis. We term this failure mode Reasoning Continuity Disruption.These observations motivate KV cache compression that jointly considers token- and reasoning-step-level information. StepKV addresses this goal by treating reasoning steps as first-class retention units. It associates cache entries with their generating steps, estimates step utility from trajectory-derived signals, and combines this utility with token-level saliency. The resulting scores globally rank prunable tokens, from which StepKV retains the top-scoring entries under a target budget. StepKV thus provides a step-centric perspective for agent KV cache compression. Across multi-hop QA and long-horizon web reasoning tasks, StepKV sustains accuracy under low KV budgets where token-level baselines degrade sharply, offering a more robust efficiency-accuracy trade-off for multi-step agent inference.

==> past_tex/relatedWork.tex <==
\section{{\color{black}Related Work}}

StepKV is related to two lines of work. The first line studies how to reduce the memory and bandwidth cost of long-context LLM inference through architectural changes, selective attention, or explicit KV cache management. The second line studies LLM agents, where inference unfolds as a trajectory of reasoning, tool use, and observations. StepKV connects these lines by asking how to compress the KV cache when the stored context is produced by an agent trajectory rather than by a single static prompt.

\subsection{LLM Agents}

LLM agents extend language-model inference from single-pass generation to interactive trajectories. Agent frameworks such as ReAct interleave reasoning and tool use through repeated Thought, Action, and Observation steps~\cite{yao2023react}; related systems use external tools, web interaction, reflection, or memory to improve task completion over multiple turns~\cite{schick2023toolformer,nakano2022webgpt,shinn2023reflexion}. This setting changes the role of context. The model is no longer conditioning only on a fixed prompt and a generated answer prefix; it also accumulates intermediate observations, retrieved evidence, and decisions whose usefulness may be delayed until later steps.

Most agent research focuses on planning, tool selection, retrieval, memory design, and benchmark performance, while the KV cache is often treated as an implementation detail of inference. Recent work has started to examine cache management for agentic inference, including model-driven, directive-based, and intent-aware approaches that decide which parts of the trajectory to retain~\cite{kariyappa2026sidequest,ma2026leyline,li2026intentkv}. StepKV is complementary to this direction: it targets the lower-level retention problem inside the KV cache and allocates a fixed cache budget using both token-level saliency and step-level utility. This distinction matters because an agent trajectory has semantic boundaries that a flat token stream does not expose; preserving those boundaries helps maintain reasoning continuity under aggressive compression.


\subsection{KV Cache Management and Compression}

KV cache optimization aims to reduce the memory and computational overhead caused by storing and accessing historical key-value states during autoregressive generation. 
Existing approaches can be broadly divided into two categories: \textbf{prefill-stage optimization} and \textbf{decode-stage KV cache management}.

\textbf{Prefill-stage optimization.}
These approaches reduce the initial cost of processing long contexts before autoregressive decoding begins. 
Grouped-Query Attention (GQA)~\cite{ainslie2023gqa} and Multi-Head Latent Attention (MLA)~\cite{deepseekai2024deepseekv2} reduce the memory footprint of KV representations by modifying the attention architecture. 
Other approaches, such as Native Sparse Attention~\cite{yuan2025nativesparse}, reduce the computation of long-context attention by selecting only relevant tokens during attention calculation. 
Meanwhile, state-space and hybrid architectures such as Mamba~\cite{gu2024mamba} and Gated Delta Networks~\cite{yang2025gateddelta} reduce the reliance on full attention for long-range dependency modeling. 
Although these methods improve long-context efficiency, they mainly optimize how representations are computed or stored during prefill and do not explicitly address which historical KV entries should be retained during evolving agent reasoning.

\textbf{Decode-stage KV cache management.}
During autoregressive decoding, the KV cache continuously grows as new tokens are generated, making selective retention necessary under limited memory budgets. 
Existing decode-stage methods mainly perform token-level cache allocation by estimating the importance of individual tokens. 
Based on the strategy used for importance estimation, these approaches can be categorized into three groups.

\textbf{Accumulated importance score-based methods.}
These methods estimate token importance using historical statistics accumulated during generation. 
H$_2$O~\cite{zhang2023h2o} identifies heavy-hitter tokens according to accumulated attention scores and preserves tokens that consistently receive high attention during decoding. 
Scissorhands~\cite{scissorhands} further studies persistent token importance by analyzing attention patterns across generation steps.
These methods effectively capture long-term token relevance but mainly rely on historical token-level statistics.

\textbf{Recent attention score-based methods.}
These approaches determine cache importance based on the attention distribution of current decoding states. 
TOVA~\cite{tova} performs online token eviction by retaining tokens that receive higher attention from recent queries. 
SnapKV~\cite{li2024snapkv} analyzes local attention patterns and preserves representative tokens from important attention regions, while Quest~\cite{quest2024} further improves cache selection through query-aware importance estimation. 
However, attention at the current decoding stage may not fully reflect the future contribution of tokens in long-horizon reasoning.

\textbf{Heuristic and structure-aware methods.}
Instead of explicitly computing token importance from attention statistics, these methods reduce KV cache through predefined rules, structural assumptions, or auxiliary signals. 
TokenSkipping~\cite{tokenskipping} periodically removes tokens according to heuristic skipping strategies, providing lightweight cache reduction without additional scoring computation. 
StreamingLLM~\cite{xiao2024streamingllm} preserves attention sink tokens and recent context based on observed attention behavior. 
Recent reasoning-oriented methods, including R-KV~\cite{cai2026rkv}, RaaS~\cite{hu2025raas}, LazyEviction~\cite{zhang2025lazyeviction}, ThinKV~\cite{ramachandran2026thinkv}, and SideQuest~\cite{kariyappa2026sidequest}, further explore redundancy-aware or reasoning-aware cache reduction strategies. 
Nevertheless, these methods still primarily operate at the token level and overlook the structured nature of agent reasoning trajectories.

\textbf{Different from existing token-centric KV cache management methods, StepKV introduces step-aware cache allocation for agent reasoning.}
Instead of treating all tokens independently, StepKV models the importance of reasoning steps and combines step-level utility with token-level saliency, enabling the preservation of critical reasoning trajectories while removing redundant context.

==> three_run_time_result.tex <==
\begin{table*}
\centering
\setlength{\tabcolsep}{4pt}
\resizebox{\linewidth}{!}{%
\begin{tabular}{ll ccc ccc ccc}
\toprule
& & \multicolumn{3}{c}{HotpotQA} & \multicolumn{3}{c}{2WikiMultihopQA} & \multicolumn{3}{c}{MuSiQue} \\
\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}
Model & Method & EM & F1 & KV Budget & EM & F1 & KV Budget & EM & F1 & KV Budget \\
\midrule
\multirow{8}{*}{Qwen2.5-7B}
& Full KV & 28.40 & 38.11 & 100 & 33.80 & 39.10 & 100 & 4.60 & 8.14 & 100 \\
& ReAct & 28.00 & 39.19 & -- & 32.60 & 38.92 & -- & 6.20 & 13.88 & -- \\
& H2O & 12.80 & 20.24 & 50 & 12.20 & 15.80 & 50 & 1.60 & 8.63 & 50 \\
& H2O &2.80  &4.64  & 20 & 1.60 & 3.42 & 20 & 0.00 & 0.52 & 20 \\
& TOVA & 11.20 & 21.40 & 50 &  10.80 & 17.42 & 50 & 1.20 & 7.75 & 50 \\
& TOVA & 1.40 & 3.63 & 20 & 2.60 & 2.23 & 20 & 0.20 & 0.46 & 20 \\
& TokenSkipping & 10.40 & 16.00 & 50 & 6.60 & 9.05 & 50 & 0.80 & 5.37 & 50 \\
& TokenSkipping & 0.20 & 0.20 & 20 & 0.00 & 0.03 & 20 & 0.00 & 0.41 & 20 \\
& StepKV (Ours) & 26.50 & 35.50 & 50 & 23.80 & 28.35 & 50 & 6.20 & 14.21 & 50 \\
& StepKV (Ours) & 19.00 & 26.26 & 20& 11.40 & 17.69 & 20& 2.40 & 9.32 & 20 \\
\midrule
\multirow{8}{*}{Llama3.1-8B}
& Full KV & 25.00 & 34.80 & 100 & 22.40 & 25.46 & 100 & 4.00 & 7.60 & 100 \\
& ReAct & 6.80 & 9.89 & -- & 6.40 & 6.93 & -- & 0.80 & 1.47 & -- \\
& H2O & 12.60 & 18.58 & 50 & 8.60 & 10.05 & 50 & 2.90 & 7.60 & 50 \\
& H2O & 0.00 & 0.57 & 20 & 0.60& 0.76 & 20 & 0.00 & 0.14 & 20 \\
& TOVA & 13.60 & 19.76 & 50 & 8.80 & 10.35 & 50 & 1.90 & 6.47 & 50 \\
& TOVA & 0.60 & 1.36 & 20 & 0.80 & 0.93 & 20 & 0.00 & 0.13 & 20 \\
& TokenSkipping & 5.20 & 8.46 & 50 & 3.80 & 5.27 & 50 & 0.60 & 4.13 & 50 \\
& TokenSkipping & 0.20 & 0.20 & 20 & 0.00 & 0.00 & 20 & 0.00 & 0.00 & 20 \\
& StepKV (Ours) & 24.00 & 37.37 & 50 & 23.20 & 26.02 & 50 & 5.10 & 10.55 & 50 \\
& StepKV (Ours) & 19.80 & 26.66 & 20 & 10.20 & 11.35 & 20 & 2.10 & 5.09 & 20 \\
\bottomrule
\end{tabular}}
\caption{Main results across datasets under different KV cache strategies run1.}
\label{tab:main_results_run1}
\end{table*}

\begin{table*}
\centering
\setlength{\tabcolsep}{4pt}
\resizebox{\linewidth}{!}{%
\begin{tabular}{ll ccc ccc ccc}
\toprule
& & \multicolumn{3}{c}{HotpotQA} & \multicolumn{3}{c}{2WikiMultihopQA} & \multicolumn{3}{c}{MuSiQue} \\
\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}
Model & Method & EM & F1 & KV Budget & EM & F1 & KV Budget & EM & F1 & KV Budget \\
\midrule
\multirow{8}{*}{Qwen2.5-7B}
& Full KV & 25.40 & 35.18 & 100 & 17.80 & 23.60 & 100 & 4.80 & 8.12 & 100 \\
& ReAct & 27.40 & 37.78 & -- & 25.00 & 31.36 & -- & 6.40 & 12.96 & -- \\
& H$_2$O & 11.40 & 19.50 & 50 & 10.40 & 14.79 & 50 & 1.80 & 7.21 & 50 \\
& H$_2$O & 1.40 & 3.25 & 20 & 0.60 & 1.98 & 20 & 0.00 & 0.96 & 20 \\
& TOVA & 9.80 & 17.57 & 50 & 8.20 & 15.92 & 50 & 2.60 &  8.29 & 50 \\
& TOVA & 0.40 & 2.65 & 20 & 0.80 & 2.08 & 20 & 0.00 & 0.33 & 20 \\
& TokenSkipping & 8.60 & 14.76 & 50 & 6.40 & 9.59 & 50 & 1.60 & 5.63 & 50 \\
& TokenSkipping & 0.40 & 0.55 & 20 & 0.00 &  0.01& 20 & 0.00 & 0.15 & 20 \\
& StepKV (Ours) &21.60  & 29.96 & 50 & 23.60 & 26.85 & 50 & 7.00 & 12.49 & 50 \\
& StepKV (Ours) & 17.60 & 23.31 & 20 & 14.40 & 16.93 & 20 & 2.60 & 6.66 & 20 \\
\midrule
\multirow{8}{*}{Llama3.1-8B}
& Full KV & 25.40 & 35.91 & 100 & 22.40 & 24.83 & 100 & 3.40 & 6.40 & 100 \\
& ReAct & 6.80 & 9.56 & -- & 4.20 & 5.03 & -- & 1.40 & 2.11 & -- \\
& H$_2$O & 10.80 & 16.24 & 50 & 8.80 & 11.93 & 50 & 3.80 & 7.27 & 50 \\
& H$_2$O & 0.80 & 1.46 & 20 & 0.60 & 0.73 & 20 & 0.20 & 0.43 & 20 \\
& TOVA & 13.20 & 17.99 & 50 & 9.40 & 11.93 & 50 & 3.60 & 6.85 & 50 \\
& TOVA & 0.60 & 1.19 & 20 & 0.40 & 0.45 & 20 & 0.00 & 0.27 & 20 \\
& TokenSkipping & 8.20 & 10.92 & 50 & 4.00 & 4.60 & 50 & 1.60 & 4.34 & 50 \\
& TokenSkipping & 0.00 & 0.00 & 20 & 0.00 &0.00  & 20 & 0.00 & 0.00 & 20 \\
& StepKV (Ours) & 25.60 & 31.60 & 50 & 21.40 & 23.91 & 50 & 4.80 & 8.93 & 50 \\
& StepKV (Ours) & 20.00 & 24.86 & 20 & 14.80 & 15.87 & 20 & 2.60 & 4.47 & 20 \\
\bottomrule
\end{tabular}}
\caption{Main results across datasets under different KV cache strategies run2.}
\label{tab:main_results_run2}
\end{table*}


\begin{table*}
\centering
\setlength{\tabcolsep}{4pt}
\resizebox{\linewidth}{!}{%
\begin{tabular}{ll ccc ccc ccc}
\toprule
& & \multicolumn{3}{c}{HotpotQA} & \multicolumn{3}{c}{2WikiMultihopQA} & \multicolumn{3}{c}{MuSiQue} \\
\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}
Model & Method & EM & F1 & KV Budget & EM & F1 & KV Budget & EM & F1 & KV Budget \\
\midrule
\multirow{8}{*}{Qwen2.5-7B}
& Full KV & 25.40 & 35.18 & 100 & 21.00 & 26.50 & 100 & 6.00 & 10.76 & 100 \\
& ReAct & 27.40 & 37.78 & -- & 25.00 & 31.03 & -- & 8.20 & 15.09 & -- \\
& H$_2$O & 11.80 & 18.97 & 50 & 9.40 & 15.29 & 50 & 2.40 & 8.56 & 50 \\
& H$_2$O & 0.40 & 2.68 & 20 & 1.00 & 2.52 & 20 & 0.00 & 1.34 & 20 \\
& TOVA & 9.20 & 18.17 & 50 & 8.60 & 14.26 & 50 & 2.00 & 8.16 & 50 \\
& TOVA & 0.40 & 2.65 & 20 & 1.00 & 2.14 & 20 & 0.00 & 1.13 & 20 \\
& TokenSkipping & 7.40 & 11.90 & 50 & 7.60 & 9.49 & 50 & 1.00 & 5.81 & 50 \\
& TokenSkipping & 0.40 & 0.43 & 20 & 0.00 &  0.19 & 20 & 0.00 & 0.00 & 20 \\
& StepKV (Ours) & 21.60 & 29.96 & 50 & 20.60 & 26.67 & 50 & 8.60 & 15.06 & 50 \\
& StepKV (Ours) & 17.60 & 23.31 & 20 & 14.60 & 18.85 & 20 & 3.40 & 8.32 & 20 \\
\midrule
\multirow{8}{*}{Llama3.1-8B}
& Full KV & 25.40 & 31.91 & 100 & 21.80 & 24.74 & 100 & 5.80 & 9.21 & 100 \\
& ReAct & 6.80 & 9.56 & -- & 4.40 & 5.25 & -- & 1.60 & 2.15 & -- \\
& H$_2$O & 12.00 & 14.72 & 50 & 8.40 & 10.94 & 50 & 2.60 & 6.78 & 50 \\
& H$_2$O & 0.80 & 1.22 & 20 & 1.40 & 2.06 & 20 & 0.20 & 0.51 & 20 \\
& TOVA & 13.20 & 17.99 & 50 & 9.60 & 11.76 & 50 & 2.00 & 6.14 & 50 \\
& TOVA & 0.60 & 1.19 & 20 & 0.60 & 0.75 & 20 & 0.00 & 0.21 & 20 \\
& TokenSkipping & 7.00 & 10.62 & 50 & 4，40 & 5.15 & 50 & 1.00 & 4.41 & 50 \\
& TokenSkipping & 0.00 & 0.00 & 20 & 0.00 &  0.00 & 20 & 0.00 & 0.00 & 20 \\
& StepKV (Ours) & 25.60 & 31.60 & 50 & 22.60 & 26.35 & 50 & 6.40 & 12.07 & 50 \\
& StepKV (Ours) & 20.00 & 24.86 & 20 & 16.40 & 18.40 & 20 & 4.40 & 7.58 & 20 \\
\bottomrule
\end{tabular}}
\caption{Main results across datasets under different KV cache strategies run3.}
\label{tab:main_results_run3}
\end{table*}
